Efficient and Effective Vocabulary Expansion Towards Multilingual Large Language Models

This report introduces \texttt{EEVE-Korean-v1.0}, a Korean adaptation of large language models that exhibit remarkable capabilities across English and Korean text understanding. Building on recent highly capable but English-centric LLMs, such as SOLAR-10.7B and Phi-2, where non-English texts are inefficiently processed with English-centric tokenizers, we present an efficient and effective vocabulary expansion (EEVE) method, which encompasses parameter freezing and subword initialization. In contrast to previous efforts that believe new embeddings require trillions of training tokens, we show that our method can significantly boost non-English proficiency within just 2 billion tokens. Surpassing most instruction-tuned LLMs on the Open Ko-LLM Leaderboard, as of January 2024, our model \texttt{EEVE-Korean-10.8B-v1.0} ranks as the leading Korean pre-trained model in the open-source community, according to Hugging Face's leaderboard. We open-source our models on Huggingface to empower the open research community in various languages.

==> bak.tex <==
% 우리는 LLM의 영어 능력을 보존한 상태에서 한국어 능력을 영어 능력에 준하는 수준으로 향상시키는 것이 목적이었다. 즉, English benchmark 에서의 성능을 베이스라인에 최대한 비슷하게 유지한 상태에서 Korean benchmark 에서의 성능을 올리는 것이 목표이다. 

% 편의를 위해 boolq, copa, hellaswag, kobest\_boolq, kobest\_copa, kobest\_hellaswag, kobest\_sentineg, kobest\_wic 

% evaluations~\cite{jang2022kobest,ko2023technical}

% \hist{open-llm-leaderboard}
% ARC, HellaSwag, MMLU, TruthfulQA, Winogrande, GSM8K

% \hist{open-ko-llm-leaderboard}
% We measured the performance on KoBEST benchmark~\cite{jang2022kobest}, on \texttt{lm-evaluation-harness}~\cite{eval-harness}\footnote{\url{https://github.com/EleutherAI/lm-evaluation-harness}}, which provides a Korean-translated version of language understanding tasks: boolean question answering (BoolQ;~\citealt{clark2019boolq}), commonsense causal reasoning (COPA;~\citealt{roemmele2011choice}, context-sensitive word understanding (WiC;~\citealt{pilehvar2019wic}), commonsense reasoning (HellaSwag;~\citealt{zellers2019hellaswag}), and sentiment negation recognition (SentiNeg). 
% \begin{itemize}
%     \item \textbf{ARC (AI2 Reasoning Challenge)}: This test evaluates scientific thinking and understanding. It measures the ability to reason necessary for solving scientific problems. It is used to assess complex reasoning, problem-solving ability, and understanding of scientific knowledge. 
%     \item \textbf{Hellaswag}: It evaluates the ability to understand and predict common situations, by testing the ability to predict the most likely next scenario in a given situation. It serves as an indicator of the models' understanding and reasoning about situations. 
%     \item \textbf{MMLU (Massive Multi-task Language Understanding)}: MMLU measures an LLM's ability to learn and apply knowledge across 57 diverse subjects including STEM, humanities, and social sciences. The test covers a wide range of difficulty levels from elementary to advanced professional. 
%     \item \textbf{Truthful QA}: It evaluates the model's truthfulness and accuracy of facts. The ability to provide truthful answers is an important criterion.
%     \item \textbf{KoCommonGEN V2}: It evaluates whether an LLM can generate Korean results that are consistent with commonsense under specific conditions.
% \end{itemize}

% \hist{As it is a Korean-translated version of an English dataset, the desired results are that the models show similar performances on both English and Korean datasets.}

% For comparison, we select the most popular LLMs with a parameter range of $\sim$13 billion: LLaMA2-13B~\cite{touvron2023llama2}, ... 

% \begin{itemize}
%     \item \textbf{SOLAR-10.7B}: A robust model incorporating Depth Up-Scaling (DUS), which includes architectural modifications and extended pre-training. Specifically, this model incorporated Mistral 7B weights into the upscaled layers and subsequently continued pre-training across the entire model.
%     \item \textbf{Phi-2}: A 2.7 billion-parameter language model that exhibits exceptional reasoning and language comprehension skills, outperforming foundational language models with less than 13 billion parameters by model scaling and sophisticated training data curation.
% \end{itemize}



% Although training a larger BPE tokenizer would enable tokenizing texts with fewer tokens, it would increase the input and output embeddings' size, resulting in more trainable parameters, which require more computational resources. 
% Furthermore, we expand the input and output embeddings by the size of our tokenizer. The newly added embeddings are randomly initialized within the space of LLamA2's embeddings. 

% Vocabulary Expansion: We meticulously selected 8,960 Korean tokens based on their frequency in our Korean web corpus. This process involved multiple rounds of tokenizer training, manual curation, and token frequency analysis, ensuring a rich and relevant vocabulary for our model.

% Training Bias Towards New Tokens: Our training data was biased to include more texts with new tokens, for effective learning. \hist{이거는 굳이 언급 안 해도 될 듯?} 

% The SOLAR-10.7B~\cite{kim2023solar}, which is an upscaled version of Mistral-7B~\cite{jiang2023mistral}, has 32,000 tokens, including only xx Korean tokens. It specifically covers Korean letters and does not include any additional Korean subwords. In this situation, fine-tuning the model with a Korean corpus can take a long time because every word is tokenized into letters. Therefore, we decide to train a new Korean tokenizer. Augmenting the SOLAR's tokenizer with Korean subwords enables fine-tuning our model on more extensive corpora within the constraints of the same computational budget. 

% Our key intuition is to best leverage the commonsense/professional knowledge and understanding/reasoning abilities of large language models, which have been shown in English, for enhancing Korean proficiency. 
% For brevity, here we describe SOLAR-10.7B~\cite{kim2023solar} as our base model, which has a vocabulary of 32,000 tokens. For Phi-1.5B~\cite{li2023textbooks}, we conduct the same process.
% For ease of explanation, we will call the newly added tokens as \textit{merged} one, and the already existing tokens as \textit{subword}, e.g., \textit{``강아지''} (merged; new) = \textit{``강''} + \textit{``아''} + \textit{``지''} (subwords; old). Sometimes, due to the BPE tokenizer~\cite{sennrich2016neural}, even the merged token could be a single character that consists of multiple bytes. 

% As a significant source of foundational capabilities for an LLM, pretraining aims to predict the next token based on the prefix sequences. Formally, given a large corpus $\mathcal{D}$, the training objective is to minimize the following loss: $\mathcal{L}_{CLM} = \sum_{x\in\mathcal{D}}\sum_{i}\log p_{\theta}(x_i|x_1,...,x_{i-1})$, where $x = \{x_1,...,x_n\}$ denotes an input token sequence tokenized by the new tokenizer. 

% Our training strategy consists of 5 distinct stages with different parameter-freezing targets, as shown in Figure. 
% stage1 - new embed\_tokens
% stage2 - new lm\_head
% stage3 - new lm\_head, new embed\_tokens
% stage4 - all lm\_head
% stage5 - all lm\_head, new embed\_tokens

% The SOLAR-10.7B~\cite{kim2023solar}, which is an upscaled version of Mistral-7B~\cite{jiang2023mistral}, has 32,000 tokens, including only xx Korean tokens. It specifically covers Korean letters and does not include any additional Korean subwords. In this situation, fine-tuning the model with a Korean corpus can take a long time because every word is tokenized into letters. Therefore, we decide to train a new Korean tokenizer. Augmenting the SOLAR's tokenizer with Korean subwords enables fine-tuning our model on more extensive corpora within the constraints of the same computational budget. 

% Hence, our approach involves training a byte-pair encoding (BPE;~\citealt{sennrich2016neural}) tokenizer with 10,000 tokens on a x GB Korean Wikipedia corpus. Furthermore, we enhance the SOLAR tokenizer by incorporating Korean subwords. The combined Korean-English tokenizer has xx,xxx tokens. Although training a larger BPE tokenized can capture more named entity tokens, it would increase the input and output embeddings' size, resulting in more trainable parameters, which requires more computational resources. Furthermore, we expand the input and output embeddings by the size of our tokenizer. The newly added embeddings are randomly initialized within the space of LLamA2's embeddings. 

% During both phases, our training objective is causal language modeling. To ensure a thorough evaluation, we divide the training into three distinct steps. 

% \subsubsection{Step 1: Pretraining to acquire language capability and knowledge}
% As a significant source of foundational capabilities for an LLM, pertaining aims to predict the next token based on the prefix sequences. Formally, given a large corpus $\mathcal{D}$, the training objective is to minimize the following loss:
% $\mathcal{L}_{CLM} = \sum_{x\in\mathcal{D}}\sum_{i}\log p_{\theta}(x_i|x_1,...,x_{i-1})$, where $x = \{x_1,...,x_n\}$ denotes an input token sequence tokenized by the new tokenizer. 

% By pretraining on massive text data ranging from billions to trillions of tokens, LLMs are capable of capturing intricate language structures, semantics, and contextual relationships, thereby acquiring strong language generation capabilities. Additionally, these LLMs also learn how to comprehend concepts, facts, and the connections between them, leading to a broad understanding of world knowledge. 

% \subsubsection{Step 2: Instruction tuning for aligning with human intent}
% Instruction tuning (SFT) aims to further enhance the capability of LLMs to follow instructions. Its training data consists of many instruction-response pairs. The model needs to learn to accurately respond to instructions, rather than merely continuing from the preceding text. Formally, given an instruction dataset $\mathcal{D}' = \{(I, Y)\}$, where $I$ represents a task instruction and $Y$ represents a desired response, the training objective of instruction tuning is to minimize the following loss:
% \begin{align}
    % \mathcal{L}_{ins}=-\log p_{\theta}(Y|I).
% \end{align}
% By tuning on diverse instruction tasks, the model is able to better comprehend and follow human instructions, and generalize to unseen instructions.

% \hist{copied from \cite{zhao2024llama}}
% \subsubsection{Extrapolating LLMs to non-English languages}
% LLMs acquire language generation and instruction-following capabilities through pretraining and instruction tuning. However, English holds a dominant position in the field of natural language processing, possessing the most abundant collection of text data from various domains. LLMs trained on English-dominant corpora exhibit inferior performance on other non-English languages. Extrapolating LLMs to non-English languages poses a highly valuable research challenge.
% Common extrapolation approaches consist of the following three steps: 
% (1) extending the vocabulary to add tokens of the target language, and thus enhancing encoding expressiveness to that language.
% (2) further pretraining to transfer language generation capabilities of LLMs to the target language. The required training scale for this step is generally on the order of billions of tokens, significantly less than the trillions of tokens needed for training from scratch.
% (3) conducting SFT in the target language to transfer instruction-following capabilities of LLMs.

% To avoid unnecessary large-scale repetitive pretraining, we employed open-source models trained on varying scales of Chinese corpora. Among these, LLaMA and LLaMA2 serve as checkpoints without undergoing explicit Chinese pretraining, whereas Chinese LLaMA and Chinese LLaMA2 are treated as checkpoints with Chinese pretraining of 30 billion tokens. The scale reaches 100 billion tokens for Open Chinese LLaMA. We employ the performance of these models as references for analysis and comparison. 


% Our strategy involved a selective freeze of model parameters. Specifically, we kept most parameters of the base model unchanged while focusing on enhancing the Korean language capabilities. Through our experiments, we discovered:

% Freezing the lm\_head layer for existing tokens is crucial to maintain overall performance.
% Unfreezing the embed\_tokens layer for existing tokens actually boosts performance.
% As a result, we froze the internal layers and the first 32,000 embed\_tokens, directing our training efforts on a rich mix of Korean and multi-lingual corpora. This balanced approach has notably improved the model’s proficiency in Korean, without compromising its original language capabilities.

% Usage and Limitations
% Keep in mind, this model hasn't been fine-tuned with instruction-based training. While it excels in Korean language tasks, we advise careful consideration and further training for specific applications.

% Training Details
% Our model’s training was comprehensive and diverse:

% Data Sources:

% English to Korean paragraph pairs: 5.86\%
% Multi-lingual corpus (primarily English): 10.69\%
% Korean web content: 83.46\%

% \hist{KoSOLAR-10.7B-v0.2 가 KoSOLAR-10.7B-v0.1 에서 바뀐 점은 lm\_head for the existing token 이 tunable 해졌다는 점. 그리고 whole parameters 가 QLoRA 를 통해 업데이트 되었다는 점.}


% Let $w_{1:T}$ be a sequence of word (identifiers) in $\mathcal{V}$, where $\mathcal{V} = \{1, ..., n\}$ is a vocabulary. Let $p_{\theta}(w_i | w_{1:i-1})$ be a natural language model parameterized by $\theta$ and defined by 
% \begin{align}
%     p_{\theta}(w_i | w_{1:i-1}) = \frac{\exp(h^{\top}_{i-1}e_{w_i})}{\sum^{n}_{j=1}\exp(h^{\top}_{i-1}e_j)},
% \end{align}
% where $h_{i-1} = \phi_{\theta}(w_{1:i-1}) \in \mathbb{R}^{d}$ is the neural representation of the prefix, and $e_i \in \mathbb{R}^{d}$ is the word embedding vector for word $i \in \mathcal{V}$. The $e_i$ are contained in $\theta$.

% In vocabulary expansion, we add a new word $n + 1 \in \mathcal{V}$. This implies we need a new word embedding $e_{n+1}$, which we sample from an \textit{initialization distribution}. The new language model, which we denote $p_{\theta'}(w_i | w_{1:i-1})$ has parameters $\theta' = \theta \cup \{e_{n+1}\} $ and is defined by
% \begin{align}
%     p_{\theta'}(w_i | w_{1:i-1}) = \frac{\exp(h^{\top}_{i-1}e_{w_i})}{Z + \exp(h^{\top}_{i-1}e_{n+1})},
% \end{align}
% where $Z = \sum^{n}_{j=1} \exp(h^{\top}_{i-1}e_j)$ is the partition function of the pre-expansion LM. 

% 머시깽이 해서 zero-initialization 을 하면 pre-expansion LM과 post-expansion LM 간의 토큰? KL divergence 가 굉장히 증가하는데, 이건 성능이 나빠진다는 뜻이다. 이걸 회피하기 위한 효율적인 방법은 새로운 단어의 embedding을 만들 때, 기존 vocab embedding의 average 로 초기화하는 것이다. 
% \begin{align}
%     & \mu = \frac{1}{n} \sum^{n}_{i=1} e_i \\
%     & e_{n+1} = \mu
% \end{align}



% \hist{from \url{https://nlp.stanford.edu/~johnhew/vocab-expansion.html}}
% In these experiments, I took 100 words that appear frequently in wikitext, but are split into multiple subword tokens by the GPT2 tokenizer. I added the words to the vocabulary of GPT2, and initialized their embeddings in three ways:
% \begin{itemize}
%     \item \textbf{default}: Use the \texttt{huggingface} default, which initializes to small random noise.
%     \item \textbf{zeros}: Initialize all new words' embeddings to the zero vector.
%     \item \textbf{avg\_emb}: Initialize using the average of all existing embeddings + small noise. 
% \end{itemize}
% I then finetuned each of four models: \texttt{gpt2-small}, \texttt{gpt2-medium}, \texttt{gpt2-large}, and EleutherAI's 125M-parameter GPT model, for 500 gradient steps, reporting the validation perplexity on Wikitext every 20 gradient steps for each initialization method. 

% So, it looks like for the \texttt{gpt2-small} and \texttt{gpt2-medium}, and \texttt{eleuther-125M} models, averaging the embeddings leads to faster adaptation to the target domain, at least as measured by perplexity on text from that domain. For \texttt{gpt2-large}, which we predict shouldn’t have a problem, we see no finetuning difference between the methods.

% \hist{Although matrix factorization itself is not new and is widely leveraged, e.g., in ALBERT (Lan et al., 2020) (a monolingual model) to lower memory consumption, we instead look at this factorization from a multilingual perspective and provide the intuition as to why such low-rank parameterization is effective in large-scale multilingual continued pretraining.}

% Given the embedding matrix $\mathbf{E}^{s} \in \mathbb{R}^{|V^{s}| \times D}$ from a source PLM that is pretrained on some source languages $S$, where $V^s$ is its subword vocabulary and $D$ is the embedding dimension, we propose to factorize the matrix ... 

% \hist{In addition, we employs parameter-efficient fine-tuning techniques~\cite{} to reduce memory consumption during model training.}


% \hist{For better reproducibility and open-source contributions, we pushed our implementations to \url{https://github.com/OpenAccess-AI-Collective/axolotl}.}

% 일단 논문에서 정리되어야 할 건 

% 1. *Pre-Training Phase*
%    - *Objective*: Enhance proficiency with existing tokens.
%    - *Method*: Continually pre-train the model using a corpus in the target language.
%    - *Focus*: Ensure maximum proficiency with the current vocabulary set.

% 2. *Base Stage: Vocabulary Resizing and Token Addition*
%    - *Objective*: Expand the vocabulary with new tokens.
%    - *Method*: Increase the size of the vocabulary and add new tokens specific to the target language.
%    - *Implementation Details*:
%      - For new tokens, inherit the output embeddings from the first subword's embeddings. This facilitates a smoother integration of new tokens using the existing knowledge base.

% 3. *Stage 1: Embedding Parameters Training*
%    - *Objective*: Train the model to understand the new tokens.
%    - *Method*: Train the model while freezing all parameters except those in embed_tokens for the new tokens.
%    - *Rationale*: By using the first subword's embeddings, this stage leverages the internal parameters already trained on the existing tokens.

% 4. *Stage 2: Language Model Head Alignment for New Tokens*
%    - *Objective*: Align the language model head (lm_head) for the new tokens.
%    - *Method*: Unfreeze and train only the lm_head parameters associated with the new tokens.
%    - *Focus*: This stage aims to align the output layer specifically for the new tokens, enhancing their representation in the model's outputs.

% 5. *Stage 3: New LM Head and Embeddings Alignment*
%    - *Objective*: Simultaneously align both lm_head and embed_tokens for the new tokens.
%    - *Method*: Train both the language model head and embeddings for new tokens, ensuring consistency and effective integration.

% 6. *Stage 4: LM Head Parameters Training*
%    - *Objective*: Enhance the overall output layer.
%    - *Method*: Freeze all parameters except the entire lm_head.
%    - *Focus*: This stage aims to refine the model's output capabilities as a whole, enhancing its generation and prediction quality.

% 7. *Stage 5: Full Model Training*
%    - *Objective*: Determine the optimal training strategy.
%    - *Method*: Unfreeze and train all model parameters.
%    - *Evaluation*: Assess the model's performance at this stage to identify the most effective snapshot (steps).

% 8. *Stage 6: Continued Pretraining with Frozen Key Components*
%    - *Objective*: Refine internal model parameters.
%    - *Method*: Freeze lm_head and embed_tokens, and continue pretraining the model's internal parameters.
%    - *Rationale*: This stage focuses on refining the deeper, internal workings of the model while maintaining the integrity of the key components related to the new tokens.

% \hist{copied from \cite{downey2023embedding}}
% Training a new SentencePiece or BPE tokenizer poses no special difficulties. However, re-initializing the embedding matrix for a new vocabulary, which will almost certainly introduce many new tokens lacking pre-trained embeddings, poses significant challenges. 

% Without loss of generality, here we consider 3 parts of LLMs: the input token embeddings (\texttt{embed\_tokens}), the output token embeddings (\texttt{lm\_head}), and the others (e.g., feed-forward layers, attentional layers). 

% Our training strategy consists of 5 distinct stages with different parameter-freezing targets, as shown in Figure. 
% stage1 - new embed\_tokens
% stage2 - new lm\_head
% stage3 - new lm\_head, new embed\_tokens
% stage4 - all lm\_head
% stage5 - all lm\_head, new embed\_tokens

% To address the poor performance of open-source LLMs in the Korean language, we introduce xxx, an open-source Korean-English LLM... 
% In this paper, we employed a Korean Byte-Pair Encoding tokenizer comprising 10,000 tokens, which has been trained on a cleaned Korean Wikipedia corpus. These tokens are added to LLaMA2's vocabulary, and the model's embeddings are subsequently expanded. We utilize the LoRA~\cite{hu2021lora} technique to train our model on a 2-billion-token Korean corpus and subsequently fine-tune the model using various instruction tuning datasets to enhance its performance on natural language processing tasks. Due to limited instruction tuning datasets for the Korean language, we refined our model by fine-tuning it on high-quality Korean machine-translated datasets. 

% a significant advancement in the field of large language models (LLMs) through the introduction of a family of Korean LLMs. Our model is built upon the foundation of two sophisticated models, SOLAR-10.7B~\cite{kim2023solar} and Phi-1.5~\cite{li2023textbooks}, which have been further pre-trained with a novel approach to vocabulary expansion specifically designed to bolster Korean language proficiency while maintaining robust performance in English. This development marks a pivotal step towards addressing the linguistic disparities often observed in LLMs, particularly between English and non-English languages.



% This technical report presents GPT-4, a large multimodal model capable of processing image and text inputs and producing text outputs. Such models are an important area of study as they have the potential to be used in a wide range of applications, such as dialogue systems, text summarization, and machine translation. As such, they have been the subject of substantial interest and progress in recent years [1–34]. One of the main goals of developing such models is to improve their ability to understand and generate natural language text, particularly in more complex and nuanced scenarios. To test its capabilities in such scenarios, GPT-4 was evaluated on a variety of exams originally designed for humans. In these evaluations it performs quite well and often outscores the vast majority of human test takers. For example, on a simulated bar exam, GPT-4 achieves a score that falls in the top 10\% of test takers. This contrasts with GPT-3.5, which scores in the bottom 10\%.

% Recent advancements in the field of large language models (LLMs) have demonstrated remarkable capabilities in processing and understanding multiple languages. Notable models such as ChatGPT~\cite{openai-gpt4}, Gemini~\cite{google-gemini}, Claude~\cite{anthropic-claude}, and LLaMA~\cite{touvron2023llama,touvron2023llama2} have set benchmarks in multilingual natural language processing. However, these developments have predominantly favored English, leading to a performance gap in non-English languages. This disparity is partly due to the inefficiency in tokenization, where languages like Korean require significantly more tokens than English for equivalent semantic content, adversely affecting both user experience and computational costs~\cite{petrov2023language}.

% The challenge of expanding LLMs' vocabulary to include more efficient tokenization for various languages has been a trade-off between improving language proficiency and maintaining the integrity of the model's original vocabulary. Traditional approaches have suggested that expanding a model's vocabulary necessitates large-scale training efforts, potentially involving trillions of tokens, to achieve stable embedding learning and prevent the dilution of the original vocabulary's representation power~\cite{zhao2024llama}. Such an approach poses significant computational costs, particularly for the open-source community, and attempts to circumvent this through parameter freezing have not fully capitalized on the model's pre-existing knowledge.

% Addressing these challenges, this paper introduces a novel vocabulary expansion technique that optimizes the balance between token efficiency and multilingual proficiency without demanding extensive computational resources. By employing distinct tokenizers for input and output sequences and initializing the output embeddings with the subword tokens from the existing tokenizer, we propose a method that allows for efficient learning of new vocab embeddings. This approach minimizes the need for extensive parameter unfreezing, thereby leveraging the model's established knowledge base and reducing the computational burden.

% Our methodology has undergone rigorous testing in both Korean and English to evaluate its effectiveness. The results indicate a significant improvement in Korean language proficiency without compromising the model's performance in English. This achievement is particularly notable given the reduced computational requirements, underscoring the potential of our approach to facilitate more efficient and effective multilingual LLM training.

% This research contributes to the ongoing efforts to enhance the accessibility and adaptability of LLMs for non-English languages, addressing the critical need for efficient pre-training methodologies. By refining the process of vocabulary expansion, our work paves the way for more inclusive language models that can serve a broader spectrum of global users, thereby enriching the diversity and specialization of LLMs across different languages.




% Recent advancements in the development and application of multilingual large language models (LLMs) such as ChatGPT~\cite{openai-gpt4}, Gemini~\cite{google-gemini}, Claude~\cite{anthropic-claude}, LLaMA~\cite{touvron2023llama,touvron2023llama2}, and other notable models like KoGPT~\cite{KoGPT2021}, Polyglot-Ko~\cite{ko2023technical}, Falcon~\cite{almazrouei2023falcon}, Mistral~\cite{jiang2023mistral}, Mixtral~\cite{jiang2024mixtral}, and Phi-1.5~\cite{li2023textbooks}, have significantly broadened the horizons of natural language processing (NLP). Despite their impressive capabilities in handling multiple languages, there's a notable proficiency bias towards English. This disparity not only hinders the effectiveness of these models in processing non-English languages but also exacerbates token inefficiency issues, leading to delayed response times and increased operational costs~\cite{petrov2023language}. Such inefficiencies are exemplified in the disparity between token requirements for English versus Korean sentences, highlighting the need for more efficient tokenization methods to bridge this gap (Figure~\ref{tab:tokenizer}).

% The exploration of vocabulary expansion as a means to enhance LLMs' language proficiency has often encountered a trade-off between efficiency and effectiveness. While expanding the vocabulary theoretically allows for better representation of diverse languages, it has historically faced challenges such as unstable embedding learning and diminished original vocabulary representation power. Conventional wisdom suggests that addressing these issues requires extensive training, sometimes up to the trillions of tokens~\cite{zhao2024llama}, posing significant computational and financial burdens, particularly for the open-source community.

% This paper introduces a novel approach to vocabulary expansion that sidesteps these challenges by leveraging existing model knowledge and optimizing training strategies for both original and expanded vocabularies. Our method involves differentiating between input and output token sequences in causal language modeling, enabling the efficient and effective incorporation of new vocabulary embeddings without extensive retraining. By utilizing a subword-based initialization strategy for output embeddings and selectively freezing and unfreezing parameters, we demonstrate that it is possible to enhance language proficiency in underrepresented languages such as Korean, without sacrificing performance in English.

% Furthermore, this study contributes to the broader discourse on developing open-source, language-specific LLMs by addressing the resource discrepancy challenge that often leaves non-English languages at a disadvantage. By efficiently transferring English-centric LLMs to support the Korean language, our work not only improves the proficiency of LLMs in processing Korean but also presents a scalable methodology that can be applied to other languages facing similar challenges.

% In doing so, this paper builds upon and extends the research landscape outlined by efforts in multilingual data mixing, cross-lingual instruction tuning, and specific initiatives like the Open Ko-LLM Leaderboard~\cite{open-ko-llm-leaderboard}, setting a new precedent for the efficient pre-training and application of LLMs across diverse linguistic contexts. Our approach represents a significant step forward in the quest to democratize access to high-quality NLP tools, ensuring that advancements in AI and machine learning are inclusive and accessible to a global user base.


% 최근 ChatGPT~\cite{openai-gpt4}나 Gemini~\cite{google-gemini}, Claude~\cite{anthropic-claude}, 그리고 LLaMA~\cite{touvron2023llama,touvron2023llama2} 등 multilingual large language models 들이 빠른 속도로 발전하고 있지만, 그들의 훈련 데이터는 대부분 영어로 구성되어 있고, non-English 언어에서의 성능은 English 에서의 성능에 비해 많이 낮은 편이다. 이 논문에서는 multilingual LLMs들의 영어 편향적인 모습에서, LLMs들의 language proficiency 측면만 볼 것이 아니라 token inefficiency 로 인해 response time 이 상대적으로 늦어지거나 API call 비용이 늘어날 수 있는 등 user experience 에 부정적인 영향을 줄 수 있다는 점을 tackle 하고자 한다~\cite{petrov2023language}. 예를 들어, Figure 1 에서 처럼 간단한 영어 문장이 LLaMA-2 tokenizer 로는 8 tokens 밖에 필요하지 않지만, 같은 뜻의 한국어 문장은 character 수가 더 적음에도 불구하고 26 tokens 이나 필요로 한다. 
% Recent advancements in multilingual large language models (LLMs) such as ChatGPT~\cite{openai-gpt4}, Gemini~\cite{google-gemini}, Claude~\cite{anthropic-claude}, and LLaMA~\cite{touvron2023llama,touvron2023llama2} have been rapid, yet their language proficiency leans towards English, leading to a significant performance disparity when compared to non-English languages. This paper addresses not only the LLMs' biased language proficiency but also the token inefficiency that can negatively impact user experience, such as delayed response times or increased API call costs~\cite{petrov2023language}. For instance, a simple English sentence may require only 8 tokens with the LLaMA-2 tokenizer, whereas a semantically equivalent Korean sentence requires 26 tokens, despite having fewer characters.

% 이런 문제를 해결하기 위해, research community 는 vocabulary expansion 을 시도해왔지만, 늘어난 vocab 을 통해 tokenization 이 효율적이게 되는 것에 비해, 1) 추가된 vocab의 embedding이 불안정하게 학습되거나, 2) 원래 vocab의 embedding이 representation power를 잃는 등 multilingual scenario에서 tokenization efficiency와 language proficiency 간의 trade-off 관계가 있어왔다. 기존의 vocab과 추가된 vocab의 token embeddings 모두를 충분히 학습시키기 위해서는 large-scale training with trillions of tokens 이 필요하다는 결과가 있어왔지만~\cite{zhao2024llama}, 이는 높은 computational cost 로 인해 open-source community 에서 감당하기가 어려운 방법이라는 단점이 있다. 더 적은 corpus 만으로도 새롭게 추가된 embeddings을 학습시키기 위해 parameter freezing 을 적용하기도 했지만~\cite{}, 모델의 기존 knowledge를 활용하지 못 하는 suboptimal 한 방법론이다. 
% Though there have been numerous researches exploring vocabulary expansion, it has faced a trade-off between tokenization efficiency and language proficiency in multilingual scenarios, where the expanded vocabularies can lead to unstable embedding learning or diminished representation power of the original vocabulary. For adequate training of both original and expanded vocab embeddings, traditional views have held that large-scale training is required up to trillions of tokens~\cite{zhao2024llama}, presenting a high computational cost challenge for the open-source community. Attempts to train new embeddings with smaller corpora through parameter freezing~\cite{} have been suboptimal, failing to utilize the model's existing knowledge. 

% 이 논문에서는, 모델의 기존 knowledge를 최대로 활용할 수 있는 vocabulary expansion 방법론을 제시한다. 우리의 핵심 가설은 causal language modeling 의 input token sequence와 output token sequence를 다르게 할 수 있다면, 모델이 새로운 vocab을 학습할 때 기존에 가지고 있던 knowledge를 최대로 활용하기 때문에 기존의 embedding space를 활용하여 새로운 vocab의 embedding 이 더 효율적/효과적으로 학습된다는 것이다. 하지만, causal language modeling 에서 input/output sequence를 서로 다른 tokenizer 로 만드는 것은 subword composition 등 구현 상의 어려움이 있다. 
% 이를 우회하기 위해, 우리는 추가된 vocab의 input embeddings (embed\_tokens) 와 output embeddings (lm\_head) 를 별개로 보고, 더 전략적으로 parameter freezing 을 시도했다. 추가된 word의 output embeddings을 이를 구성하는 subword 의 output embeddings 로 initialization 함으로써, 우리는 input/output token sequence를 동일하게 유지하면서도 모델이 학습 과정에서 기존 vocab의 embeddings space 에 새로운 단어들의 embeddings 를 효과적으로 align 되도록 하였다. 
% This paper presents a novel vocabulary expansion method that fully leverages a model's pre-existing knowledge. Our principal hypothesis is that if the input and output token sequences in causal language modeling can be differentiated, the model can more efficiently and effectively learn new vocab embeddings by leveraging its established knowledge and embedding space. However, employing distinct tokenizers for input and output sequences poses implementation challenges, such as the difficulty of applying teacher forcing due to mismatched input/output sequences. To circumvent these challenges, we provide a proxy of \texttt{token\_ids} by introducing a subword-based initialization of output embeddings (\texttt{lm\_head}). As described in Figure 2, we freeze most of the parameters except the input embeddings (\texttt{embed\_tokens}) of newly expanded tokens, while initializing the output embeddings \texttt{lm\_head} with that of its first subword token from the old tokenizer. In this way, we could give feedback on the model to generate the subword token (old) given the merged token (new). On the other hand, the model could learn to align the representation for generating the merged token with that for the first subword token, by optimizing only \texttt{embed\_tokens} without any modification of input/output token sequences. Afterward, we gradually unfreeze the parameters, eventually leading to the model being fully trained.
% As described in Figure 2, if the new token (merged) shares the \texttt{lm\_head} of its subword token from the old tokenizer, where  the model could learn to align the tokens in compositional relationships, without modifying input/output token sequences.
% separately consider the input embeddings (\texttt{embed\_tokens}) and output embeddings (\texttt{lm\_head}) of the expanded vocabulary, strategically applying parameter freezing. By initializing the output embeddings of new words with those of their constituent subwords, we maintain identical input/output token sequences while aligning new word embeddings effectively within the existing vocab's embedding space. \hist{설명이 살짝 부족한 것 같다. 어려움.}

% 우리는 여러 benchmark datasets 에서 우리의 training strategy 가 기존 vocabulary expansion 방법론들의 token efficiency 개선 효과 뿐만 아니라, 한국어에서의 language proficiency 까지도 효율적으로/효과적으로 개선할 수 있음을 경험적으로 보였다.
% To verify the effectiveness of our training strategy, we conducted evaluations in both Korean and English. From the results, we found that our method could significantly enhance language proficiency in Korean, while preserving strong results in English. It is noteworthy that we could get such performance improvements with fewer computational resources, due to the more efficient tokenization of expanded vocabulary, which affects the overall process of training language models, by decreasing the token sequence length. 

% Our key contributions are as follows:
% \begin{itemize}
%     \item We introduce a novel strategy for vocabulary expansion based on embedding initialization and parameter freezing. 
%     \item We achieve top performance in KoBEST~\cite{jang2022kobest} dataset, while preserving strong results of the base model in English datasets. 
%     \item We 
% \end{itemize}
% Empirical evidence from various benchmark datasets demonstrates that our training strategy enhances language proficiency in Korean, while keeping the advantages of vocabulary expansion, token efficiency, showcasing its effectiveness and efficiency. 


% 우리는, Figure 2에서 볼 수 있듯이, next token prediction 이라는 목적을 재해석해, $i-1$번째 토큰까지 입력으로 들어왔을 때, 기존 vocab에 속하던 $x^{old}_i$ 토큰이 아니라 vocab에 새로이 추가된 $x^{new}_i$ 토큰을 생성할 수 있도록 하는 것에 집중했다. 

% Our distinct intuition is that input/output token embeddings 를 별개로 보고, parameter freezing을 전략적으로 시도함으로써, 
% 기존 vocab의 embeddings을 유지하기 위해 parameter freezing 을 하고, 새롭게 추가된 vocab의 embeddings 를 우선적으로 
% Our distinct intuition 은 parameter freezing 을 통해 기존 vocab의 embeddings을 유지하면서 새롭게 
% an approach that is beyond the reach of many in the open-source community due to its high computational cost.
% 구성되어 있기 때문에 non-English 언어에서의 성능은 English 에서의 proficiency에 비해 많이 낮은 편이다. ChatGPT나 Gemini 같은 proprietary LLMs 들은 English 외에도 좋은 성능을 보여주는 편이지만, open-source LLMs 에서는 그들의 성능이 더더욱 English 에 치우처져 있는 편이다. 최근 multilingual LLMs 들이 공개되고는 있지만, 이들은 대부분 English 와 Chinese 데이터셋에서 학습된 모델들이고, Korean 에서는 KoGPT, Polyglot-Ko 등이 있었으나 최근 LLMs 에 준하는 open-source models 은 없었다. 그리고 이런 open-source LLMs의 language proficiency 뿐만이 아니라, token efficiency 또한 multi-lingual LLMs 의 중요한 문제임을 argue 한다.

 

% However, these models not only underperform in non-English languages, but also 
% but these models often underperform in non-English languages due to their primary training on English data.
% This not only highlights a gap in achieving language proficiency equality across multiple languages but also raises concerns due to the tokenizers these models employ being optimized for English. 
% However, these models, including notable ones such as LLaMA~\cite{touvron2023llama,touvron2023llama2}, often underperform in languages other than English due to their primary training on English data. This not only highlights a gap in achieving language proficiency equality across multiple languages but also raises concerns due to the tokenizers these models employ being optimized for English. 
% As a result, when processing languages like Korean, which this paper focuses on, the ratio of tokens to characters increases significantly. This leads to longer token sequence length, which negatively affects computational costs and response times, presenting substantial challenges in efficiently extending the capabilities of LLMs to non-English languages, which we named as efficiency-equality trade-off. % token efficiency 와 language proficiency equality 간의 trade-off 에 대한 논의가 있어왔다.

 
% However, vocabulary expansion has seemed to hinder language transferability, requiring a large-scale pre-training with trillions of tokens to be effective~\cite{zhao2024llama}.

% Here we thus argue for its necessity 
% \hist{vocab expansion 이 성능에 좋지 않은 영향을 끼친다는 여러 분석이 있었으나, vocab expansion 을 통한 non-English languages 에 대한 overall inference speed 향상을 고려했을 때, vocab expansion 은 practical use of LLMs 를 위한 필수 요소로서 고려되어야 한다.}
% \hist{copied from \cite{zhao2024llama}} In the previous section, we observed that extending the vocabulary had a negative impact on language transferability. A plausible hypothesis is the existence of cross-lingual semantic alignment within LLMs, which vocabulary expansion might disrupt. 
% Addressing this issue, our study introduces an innovative method focused on expanding the vocabulary of these models in a way that significantly enhances their understanding of multiple languages with a smaller dataset, specifically just 2 billion tokens. Traditional views have held that expanding a model's vocabulary to effectively support multiple languages required training with trillions of tokens, an approach that is beyond the reach of many in the open-source community due to its high computational cost.

% Despite previous analyses suggesting that expanding the vocabulary might negatively impact a model's ability to transfer knowledge across languages, our method proves otherwise. By smartly initializing the embedding tokens and adjusting the model with a layer-freezing schedule, we align new and existing vocabularies efficiently. This process not only preserves the model’s performance in English but also bridges the gap in its ability to understand and generate text in other languages.

% Our approach is strategic, starting with enhancing the model’s grasp of existing vocabulary through initial training phases. Then, we move to a crucial stage of adding new, language-specific tokens, aiming to incorporate these seamlessly into the model’s existing knowledge base.

% This paper also tackles the often-ignored issue of maintaining performance in English while boosting proficiency in other languages. Through our meticulously planned stages of vocabulary expansion and targeted training, we ensure an improvement in non-English language skills without compromising the model's English capabilities.


% In the rapidly evolving field of large language models (LLMs), achieving multilingual proficiency remains a significant challenge. 
% While LLMs demonstrate remarkable proficiency in English, their performance in other languages often lags. 
% This paper introduces a comprehensive methodology aimed at bridging this proficiency gap, focusing on strategic vocabulary expansion and targeted training stages. 
% \hist{recently LLMs quickly have evolved, even performing better than humans, but their performances in non-English languages are reportedly worse than that in English. Though some LLMs are developed for either English or other languages, such as Bard in Korean, there are still gaps between proprietary LLMs and open-source LLMs. In the open community, LLaMA-2~\cite{touvron2023llama2} has been actively studied and many of the top-performing LLMs in HuggingFace open-llm-leaderboard are based on LLaMA-2. 걔네의 성능은 proprietary LLMs 의 다른 언어 능력들보다 떨어진다. }
% \hist{그리고 이 논문에서는 open community 의 limited computation resource를 고려하여 13B 이하의 LLM 들만 고려하였다. }
% \hist{recently, LLM은 multi-lingual language models 로서 동작한다. 하지만, 기존 cross-lingual language models에 비해 wider coverage for languages 를 보여주지만, English와 non-English languages 간에는 여전히 엄청난 performance gap 이 존재한다~\cite{...}.}
% \hist{vocab expansion 이 성능에 좋지 않은 영향을 끼친다는 여러 분석이 있었으나, vocab expansion 을 통한 non-English languages 에 대한 overall inference speed 향상을 고려했을 때, vocab expansion 은 practical use of LLMs 를 위한 필수 요소로서 고려되어야 한다.}
% \hist{copied from \cite{zhao2024llama}} In the previous section, we observed that extending the vocabulary had a negative impact on language transferability. A plausible hypothesis is the existence of cross-lingual semantic alignment within LLMs, which vocabulary expansion might disrupt. 
% \hist{법적 이슈로 인해 web corpus 를 함부로 사용하는 것이 부담스러울 수 있다.}
% \hist{From Orion-14B tech report}
% The launch of ChatGPT/GPT3.5 in 2022 captured tremendous attention from the public, pushing the boundaries of what AI can achieve and motivating researchers and engineers to delve deeper into their potential. While GPT-3.5 and its successor, GPT-4 are prime examples of LLMs, their specific model architectures and training methodologies remain undisclosed. In contrast, Meta's release of LLaMA~\cite{touvron2023llama} and LLaMA 2~\cite{touvron2023llama2} have established a widely-recognized LLM architecture within the open-source community, with numerous libraries adopting these models. Despite LLaMA's impressive performance, its primary focus on English limits its applicability to other languages. Recently, there has been a surge in the release of multilingual LLMs such as ChatGLM, Baichuan, Qwen, InternLM, XVERSE, Skywork, and Yi. These models, trained on mainly English and Chinese datasets, have shown promising results in tasks involving both English and Chinese. Additionally, there has been a growing trend of LLMs specifically designed to enhance performance in other languages, such as Japanese and Korean.


% \hist{심지어, as it uses BPETokenizer~\cite{sennrich2016neural}, it is reportedly very slow to tokenize the Asian texts, such that consuming 3 tokens to process a single character. inefficient tokenization 은 input token sequence 의 길이를 늘리고, Transformers 아키텍쳐는 이를 quadratic 한 computation 을 필요로 하기 때문에, non-English language researchers 들에게 굉장한 resource 부담감과 불편함을 주게 된다. To tackle this issue, vocab expansion 방법론이 연구되었으나, 이는 보통 a large size of pre-training corpus 를 요구하기 때문에, 그 자체로 computationally expensive 한 작업이었고, 심지어 몇몇 최근 연구에서는 이 방법이 기존의 모델을 0.5B token 으로 fine-tuning 하는 것보다 오히려 성능이 떨어진다는 분석도 있었다~\cite{zhao2024llama}. 즉, token efficiency 와 language understanding ability 간의 trade-off 가 있다는 것이다. }
% \hist{Initially, we collected one million Chinese sentences from the internet (approximately 0.5 billion tokens) and further pretrain the original LLaMA without vocabulary extension. Surprisingly, we find that this model significantly outperform the vocabulary-extended Chinese LLaMA, across settings of 1K, 5K, and 950K instruction tuning. This discovery is thought-privoking, given that the Chinese LLaMA underwent further Chinese pretraining on 30 billion tokens, a much larger volume than our 0.5 billion tokens. }

% Initially, the pre-training phase enhances proficiency with existing tokens. By continually pre-training the model using a corpus in the target language, we aim to maximize proficiency with the current vocabulary set. This foundational stage sets the stage for more advanced vocabulary and model adjustments.

% Following this, we initiate the Base Stage of vocabulary resizing and token addition. The objective here is to expand the model's vocabulary with new, language-specific tokens. Implementing this involves increasing the vocabulary size and integrating new tokens by inheriting output embeddings from the first subword. This approach facilitates a smoother integration of new tokens, leveraging the existing knowledge base.




% \hist{need to draw a figure: embed\_tokens, lm\_head, internal layers, LoRA}
% \hist{우리도 solar 모델 하나만으로는 너무 부족한 것 같아서 phi-2 돌려봤고, 서로 다른 tokenizer (SOLAR 는 LlamaTokenizer, Phi-2는 CodeGenTokenizer) 를 사용했음에도 불구하고, 똑같이 significant 한 성능 향상을 확인할 수 있었다}

% Our contributions can be summarized as follows:
% \begin{itemize}
%     \item 1. We propose a practical approach that can significantly improve the non-English performance of LLMs, by revisiting the vocab expansion approach.
%     \item 2. We propose a novel approach to initializing the embeddings of newly expanded tokens. 
%     \item 3. We publicly released our model for accelerating the Korean LLM researches. 
% \end{itemize}


% Expanding the existing tokenizer with Korean subwords would enable training the models on more extensive corpora within the constraints of the same computational budget. Our key claim, in contrast with common beliefs that new embeddings require trillions of training tokens~\cite{zhao2024llama}, is that it can be achieved with only several billions of tokens. Similar problems have already been considered recently~\cite{rostami2024persianmind,guo2023owl}, to the best of our knowledge, but this work is the first to transfer LLMs to other languages without loss of English proficiency. 

% on finding a resource-efficient way of further pre-training LLMs on Korean texts with vocabulary expansion. Though there have been beliefs that new token embeddings require trillions of training tokens~\cite{zhao2024llama}, here we focus on developing 
% Though vocabulary expansion and parameter-freezing is not entirely novel~\cite{rostami2024persianmind,guo2023owl}, 
% Our focus is on developing a novel parameter-freezing method for resource-efficiently expanding the vocabulary with non-English tokens. 
% Though there have been related efforts of adopting parameter-freezing, introducing additional tokens in Persian~\cite{rostami2024persianmind} and language-specific experts, \hist{바꿔야함}
% These methods are inspired by successful strategies in similar contexts, such as the incorporation of additional subword tokens in LLaMA2 for improved language understanding, as discussed in related research~\cite{rostami2024persianmind}, and the application of language-specific training experts with pre-trained weight freezing, a concept explored by \cite{guo2023owl}.

% By adopting these techniques, we contribute to the ongoing discussion on how to effectively bridge the resource gap in LLMs for non-English languages. Our approach seeks to enhance the representation and performance of the Korean language within the LLM ecosystem, offering insights into the potential for language-specific model training.

% This paper focuses on the development of Korean-specialized open large language models (LLMs) such as KoGPT~\cite{KoGPT2021} and Polyglot-Ko~\cite{ko2023technical}, amidst the broader landscape of commercial and open-source LLMs that exhibit varying capabilities in multilingual support. While models like GPT-4~\cite{openai-gpt4}, PaLM2~\cite{anil2023palm}, Gemini~\cite{google-gemini}, and Claude~\cite{anthropic-claude} have demonstrated proficiency in multiple languages, their proprietary nature often restricts access and fine-tuning. 
% Open-source alternatives, including LLaMA2~\cite{touvron2023llama2}, Falcon~\cite{almazrouei2023falcon}, Mistral~\cite{jiang2023mistral}, Mixtral~\cite{jiang2024mixtral}, and Phi-1.5\cite{li2023textbooks}, show promise in English but face limitations in broader language coverage, with efforts like Orion-14B~\cite{chen2024orion} attempting to address this gap albeit with limited success in non-English languages. 
% \hist{fine-tuning 기깔나게 하고있지 요즘 instruction tuning \cite{chung2022scaling}, preference tuning~\cite{bai2022training,ouyang2022training,rafailov2023direct}}

% Despite the existence of numerous models, the recent unveiling of the Open Ko-LLM Leaderboard~\cite{open-ko-llm-leaderboard} highlighted the proliferation of models with a specific focus on Korean language enhancement. Prior efforts largely concentrated on fine-tuning existing pretrained models for Korean instructions, revealing a gap in the development of fundamentally Korean-centric LLMs. This paper aims to elevate the proficiency bar of open LLMs in Korean by exploring efficient and effective methods for training Korean LLMs, thus contributing to the diversification and specialization of open-source LLMs.

% \hist{copied from \cite{zhao2024llama}}
% One of the main challenges of LLMs is the resource gap, as they are mainly pretrained on English corpus and have limited access to data from other languages. 
% This creates a disparity in language models' capability to handle different languages. 
% Previous findings indicate that LLMs have difficulty comprehending and generating non-English texts, particularly in low-resource languages. 

% Though there are numerous attempts to enhance language proficiency in multilingual language models, such as LoRA~\cite{hu2021lora} 나 adapter 를 통한 parameter-efficient training 방법론들이 있지만, 우리는 embedding layers 의 parameter freezing 과 embedding initialization strategy를 통한 parameter-efficient training 을 탐구했다. data mixing 도 있고... \cite{zhu2023extrapolating} 처럼 cross-lingual instruction tuning 도 있고. 그 중에서도, pre-training 을 할 거고, vocab expansion 을 통해 practical usage 도 고려한다. language-adpative pre-training (LAPT) Language-Adaptive Pre-Training (LAPT)--continunig the MLM or CLM pre-training task on only the target language(s)-- is a simple and strong baseline in this regard. 다만 parameter freezing 을 통해 pre-training 단계에서 vocab expansion 을 하는 것은 우리가 처음? 

% Extensive work has proposed re-using and modifying pre-trained models for new settings in order to retain existing model knowledge and reduce pre-training costs. \cite{gururangan2020don} show that continued training on domain-specific data effectively adapts pre-trained models to new domains in both high- and low-resource settings. 
% Research transferring monolingual models from one language to another has shown that random re-initialization of embeddings + LAPT is sufficient. 
% 확장 방법론


% \cite{downey2023embedding} 반면에 이 논문은 multilingual models 의 vocab 이 너무 커져서 computational cost 의 문제나 under-optimization 의 문제를 다루기 위해 vocab을 더 compact 하고 language-specific 한 것으로 바꾸는 것을 시도한다. 

% The alternative way is to use publicly available multilingual PLMs as the source models and continued pretrain them on a set of target languages. This continued pertaining approach is in favor because it consumes fewer resources than training from scratch, which is important when the computation budget is limited given the continually increasing model size. 

% non-English language 를 위한 data-centric 연구들이 있었으나~\cite{chung2023unimax,ogunremi2023mini} 우리 논문에서는 training algorithm 을 다룬다.

% Recent efforts to cover these languages instead pre-train models that are specialized to specific languages or language families. 
% These approaches nonetheless require training a new model from scratch and do not leverage transferable information in existing models. 
% However, LAPT with no change to the cross-lingual vocabulary comes with considerable excess computational cost: when adapting to a single language or small subset of languages, only a small fraction of the cross-lingual vocabulary is used. The excess vocabulary still contributes to the computational cost on both the forward and backward pass, and embedding/output matrices often constitute a large fraction of the total trainable model parameters (for XLM-R-base, 192M / 278M $\simeq$ 69\% of parameters). Additionally, the information-theoretic tokenization modules for cross-lingual models are usually under-optimized for any given language, and especially low-resource languages. 

% A major limitation in adapting pre-trained models to new languages is the subword vocabulary, which often fails to cover an unseen script or tokenizes target text inefficiently. When transferring a monolingual model to a new language, xxx instead completely re-initialize the embedding matrix, corresponding to a new subword vocabulary. These embeddings are then trained into alignment with the pre-trained, frozen transformer encoder. 

% Other work reuses information in pre-trained embeddings rather than initializing new ones at random. This may include scaling up smaller embedding spaces from models trained on the target language or copying embeddings from the original vocabulary where there is exact vocabulary overlap. 


% To preserve whitespace information, SentencePiece tokens include a leading underscore to indicate tokens that should be preceded by a space (word-initial tokens). 

% \hist{copied from \cite{si2023empirical}}
% Comparison of Parameter-efficient Methods. From Table 4, several observations can be derived: 1) SadapterH performs the best among all parameter-efficient methods, which can be used as an alternative to LoRA. 2) P-tuning and prompttuning underperform others by large margins, indicating that only adding trainable layers in the embedding layer are not enough to support LLMs for generation tasks. 3) Although AdaLoRA is an improvement of LoRA, its performance has a clear drop, possibly because the LoRA’s trainable parameters for LLMs are not suitable for further reduction. 4) Comparing the upper and lower parts, it can be seen that increasing the number of trainable parameters for sequential adapters (i.e., SadapterP and SadapterH) does not bring gain, while the opposite phenomenon is observed for parallel adapters (i.e., P-adapter). This may provide inspiration for the design of adapters for LLM. Since LoRA is currently the most popular parameter-efficient method, if not otherwise specified, we adopt LoRA by default in the experiments.

% \hist{\href{https://stability.ai/news/introducing-stable-lm-2}{Stable LM2} 의 발표에 따르면 걔네는 2 trillion tokens 를 2 epochs 이나 돌렸다고 한다. 지구한테 사과해라.}\
% \hist{copied from \cite{chen2024orion}}
% Pretraining of LLM needs tremendous amounts of data. \cite{hoffmann2022training} offered guidelines regarding the optimal quantity of training data for models of varying sizes. For example, an LLM with 10 billion parameters requires 205 billion tokens for pretraining. However, recent work in training 10 billion parameter models have utilized 2.5 to 3 trillion tokens, substantially exceeding the recommended data volume. These efforts have yielded notably impressive results, demonstrating the efficacy of training with significantly larger datasets than those proposed in the aforementioned study.


 % BPE tokenizer~\cite{sennrich2016neural}

% Korean: HyperCLOVA (82B GPT3)~\cite{kim2021changes,shin2022effect}, 

% \hist{vocab expansion 할 때 just average all existing embeddings to initialize new embeddings 를 하는 경우가 있음. 이걸 베이스라인으로 고려해야 할 것 같다}

% \mh{\cite{chung2023unimax}는 multilingual pretraining에서 high-resource language와 low-resource language 사이의 imbalance를 문제로 제기했다. 일반적인 해결방법인 temperature 기반 upsampling의 경우, low-resource language의 적은 sample들이 과하게 반복되는 문제가 있었다. 이를 해결하기 위해, unimax라는 접근법을 제안했다. 구체적으로는, 모든 학습 대상 언어를 동일한 character 만큼 학습할 수 있도록 각 언어별로 character budget을 지정한다. 다만, low-resource language가 과하게 반복되는 현상을 막기 위해 최대 반복 횟수 N을 지정하여 이 이상 등장할 수 없게 한다. 이 논문은 low-resource language에 overfitting 되는 것을 방지하는 방법을 제시하나, 여전히 모델을 학습할 때 대량의 토큰을 보아야만 한다는 단점이 있다.}

% \mh{\cite{ogunremi2023mini}는 multilingual pretraining에서 모델이 더 많은 언어들을 학습하면 학습할수록 target으로 하는 low-resource language에 대한 능력이 희석됨을 문제로 제기하였다. 실제로, low-resource language에 속하는 African 계열 언어에 대해서, massive language model보다 약 1GB 정도의 데이터로 scratch부터 학습한 AfriBERTa가 target language의 downstream task에서 훨씬 뛰어난 성능을 보였다. 이 논문에서는 이 방향을 확장하여, 보다 적은 양의 low-resource language만 가지고 뛰어난 성능을 얻는 법에 대해 탐구한다. low-resource language를 학습할 때, 해당 언어와 언어학적으로 유사한 family를 함께 학습 할 경우 훨씬 적은 양의 데이터만으로 comparable한 성능을 얻을 수 있음을 확인하였다. 이 논문은 low-resource language를 scratch부터 효과적으로 학습하는 방법을 제시하나, massive language model의 knowledge를 활용할 수 없다는 단점이 있다. -> 우리 방법론은 기존 massive language model의 knowledge와 low-resource langauge를 align 시킨다는 차별점이 있다.}

==> figure_latex/freezing.tex <==
\begin{figure}[h]
\centering
\begin{lstlisting}[language=Python]
def freeze_partial_embedding_hook(grad):
    grad[:32000] = 0
    return grad

for name, param in model.named_parameters():
    if ("lm_head" in name or "embed_tokens" in name) and "original" not in name:
        param.requires_grad = True
        if "embed_tokens" in name:
            param.register_hook(freeze_partial_embedding_hook)
    else:
        param.requires_grad = False
\end{lstlisting}
\caption{Python code for freezing partial embeddings}
\label{fig:freezing}
\end{figure}

==> table_latex/ablations.tex <==
\begin{table}[t]
  \centering
  % \small % or \footnotesize for smaller size
  \resizebox{0.98\columnwidth}{!}{
  \begin{tabular}{@{}lccccccccc}
  \toprule
  \multirow{3}{*}{Model} & \multicolumn{3}{c}{English} & \multicolumn{5}{c}{Korean} \\ \cmidrule(l){2-4} \cmidrule(l){5-9} 
   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BQ \\ (0)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}CP \\ (0)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}HS \\ (0)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BQ \\ (0)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}CP \\ (0)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}HS \\ (0)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SN \\ (0)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}WIC \\ (0)\end{tabular}} \\ \\ \midrule
  Stage 0 & 0.8336 & 0.9000 & 0.5583 & 0.5021 & 0.4770 & 0.3280 & 0.5063 & 0.4881 \\ \midrule
  Stage 1 & 0.8336 & 0.8900 & 0.5536 & 0.5021 & 0.4720 & 0.2240 & 0.4962 & 0.4881 \\ 
  Stage 2 & 0.8339 & 0.9000 & 0.5540 & 0.5021 & 0.4790 & 0.2100 & 0.4962 & 0.4881 \\ 
  Stage 3 & 0.8373 & 0.9000 & 0.5539 & 0.5021 & 0.4900 & 0.2080 & 0.4962 & 0.4881 \\ 
  Stage 4 & 0.8361 & 0.8800 & 0.5564 & 0.5021 & 0.4790 & 0.2120 & 0.4962 & 0.4881 \\ 
  Stage 5 & & & & & & & & \\ 
  Stage 6 & & & & & & & & \\ 
  Stage 7 & & & & & & & & \\ 
  \bottomrule
  \end{tabular}
  }
  \caption{Ablation studies per stages. Note that ``Stage 0'' and ``Stage 7'' denote the base model and our final model, microsoft/Phi-2 and yanolja/EEVE-Korean-2.7B-v1.0 respectively.}
  \label{tab:ablation-studies}
\end{table}

==> table_latex/stages.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|cc|cc|c}
    \toprule
    \multirow{2}{*}{Stage} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\texttt{embed\_tokens}\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\texttt{lm\_head}\end{tabular}} & \multirow{2}{*}{\texttt{layers}} \\ 
    \cmidrule{2-3} \cmidrule{4-5}
     & Old & New & Old & New & \\
    \midrule
     0 & \emoji{snowflake} & \emoji{snowflake} & \emoji{snowflake} & \emoji{snowflake} & \emoji{snowflake} \\ \midrule
     1 & \emoji{snowflake} & \emoji{fire} & \emoji{snowflake} & \emoji{snowflake} & \emoji{snowflake} \\
     2 & \emoji{snowflake} & \emoji{snowflake} & \emoji{snowflake} & \emoji{fire} & \emoji{snowflake} \\
     3 & \emoji{snowflake} & \emoji{fire} & \emoji{snowflake} & \emoji{fire} & \emoji{snowflake} \\
     4 & \emoji{snowflake} & \emoji{fire} & \emoji{fire} & \emoji{fire} & \emoji{snowflake} \\
     5 & \emoji{snowflake} & \emoji{snowflake} & \emoji{snowflake} & \emoji{snowflake} & \emoji{fire} \\
     6 & \emoji{fire} & \emoji{fire} & \emoji{fire} & \emoji{fire} & \emoji{fire} \\
    \bottomrule
    \end{tabular}
    \caption{Training stages with parameter freezing}
    \label{tab:stages}
\end{table}
